Style Equalization: Unsupervised Learning of Controllable Generative Sequence Models

Controllable generative sequence models with the capability to extract and replicate the style of specific examples enable many applications, including narrating audiobooks in different voices, auto-completing and auto-correcting written handwriting, and generating missing training samples for downstream recognition tasks. However, under an unsupervised-style setting, typical training algorithms for controllable sequence generative models suffer from the training-inference mismatch, where the same sample is used as content and style input during training but unpaired samples are given during inference. In this paper, we tackle the training-inference mismatch encountered during unsupervised learning of controllable generative sequence models. The proposed method is simple yet effective, where we use a style transformation module to transfer target style information into an unrelated style input. This method enables training using unpaired content and style samples and thereby mitigate the training-inference mismatch. We apply style equalization to text-to-speech and text-to-handwriting synthesis on three datasets. We conduct thorough evaluation, including both quantitative and qualitative user studies. Our results show that by mitigating the training-inference mismatch with the proposed style equalization, we achieve style replication scores comparable to real data in our user studies.

==> table_handwriting.tex <==

\begin{wraptable}{r}{0.38\textwidth}
	\vspace{-6mm}
	\caption{{Handwriting results}}
	\label{table: handwriting}
	\small
	\def\tablewidth{18mm} 
	\centering
	\setlength{\tabcolsep}{2pt}
	\vspace{-2mm}
	\begin{adjustbox}{max width=\linewidth}
		\begin{tabular}{p{19mm}rrr}
			\toprule
			\multirow{2}[3]{*}{Method} & 
			\multicolumn{1}{c}{parallel text}  &   
			\multicolumn{2}{c}{nonparallel text}  
			\\ 
			\cmidrule(lr){2-2} \cmidrule(lr){3-4} 
			& 
			\multicolumn{1}{c}{CER (\%)}  &
			\multicolumn{1}{c}{CER (\%)}  & 
			\multicolumn{1}{c}{opinion score}
			\\
			\midrule
			\cite{graves2013generating}& 
			$13.6 \pm 0.9$ & 
			$17.7 \pm 1.7$ &   
			$2.7 \pm 0.9$ 
			\\
			No-SEQ & 
			$5.9 \pm 1.2$ &   
			$69.8 \pm 2.3$ &  
			$1.5 \pm 0.6$
			\\
			\midrule
			Proposed  & 
			$\mathbf{3.3 \pm 0.2}$  & 
			$\mathbf{5.5 \pm 1.2}$ &  
			$\mathbf{3.4 \pm 0.6}$
			\\
			\midrule
			Same writer &
			$2.7 \pm 0.7$   &  
			$2.7 \pm 0.7$ & 
			$3.4 \pm 0.8$
			\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{wraptable}




==> table_speech.tex <==

\begin{table}
	\caption{\textbf{Experiment results --- speech (VCTK), parallel text.} The table shows the quantitative evaluation results on VCTK dataset. In the experiment, the style references are drawn from the training set (seen speakers) and have the same content from the target content. }
	\label{table: vctk, train, parallel}
	\def\tablewidth{18mm} 
	\centering
	\begin{tabular}{p{47mm}C{\tablewidth}C{\tablewidth}C{\tablewidth}C{\tablewidth}}
		\toprule
		Method     & Word-error rate (\%) $\downarrow$  \newline (real: 7.8)  &  Cosine \newline similarity $\uparrow$  &  Mean opinion score (naturalness) $\uparrow$ &  Mean opinion score (similarity) $\uparrow$ \\
		\midrule
		Tacotron & $12.8$ & $0.18 \pm 0.17$  & \todo{}  & \todo{}   \\
		GST (\# tokens = 16)  & $19.6$ &  $0.25 \pm 0.14$ & \todo{}  & \todo{}   \\
		GST (\# tokens = 64)  & $6.6$  & $0.29 \pm 0.16$  & \todo{}  &  \todo{}  \\
		GST (\# tokens = 16)  + embedding  &  $4.5$ & $0.46 \pm 0.12$ & \todo{} & \todo{}    \\
		GST (\# tokens = 64) + embedding & $7.2$ & $0.45 \pm 0.12$ & \todo{} & \todo{}   \\
		Proposed (dim knobs = 64) & $7.9$ & $0.68 \pm 0.14$ & \todo{}  & \todo{}  \\
		\bottomrule
	\end{tabular}
\end{table}

\begin{table}
	\caption{\textbf{Experiment results --- speech (VCTK), nonparallel text.} The table shows the quantitative evaluation results on VCTK dataset. In the experiment, the style references are drawn from the training set (seen speakers) and have different contents from the target contents. }
	\label{table: vctk, train, nonparallel}
	\def\tablewidth{18mm} 
	\centering
	\begin{tabular}{p{47mm}C{\tablewidth}C{\tablewidth}C{\tablewidth}C{\tablewidth}}
		\toprule
		Method     & Word-error rate (\%) $\downarrow$  \newline (real: 7.8) &  Cosine \newline similarity $\uparrow$  &  Mean opinion score (naturalness) $\uparrow$ &  Mean opinion score (similarity) $\uparrow$ \\
		\midrule
		Tacotron & $14.3$  & $0.01 \pm 0.14$  &  \todo{} & \todo{}   \\
		GST (\# tokens = 16)  & $22.3$  & $0.26 \pm 0.18$  & \todo{}  & \todo{}    \\
		GST (\# tokens = 64)  & $29.5$  & $0.23 \pm 0.16$  &  \todo{}  &  \todo{}   \\
		GST (\# tokens = 16)  + embedding  & $21.0$  & $0.29 \pm 0.16$  &  \todo{}  &  \todo{}   \\
		GST (\# tokens = 64) + embedding & $24.8$  & $0.33 \pm 0.17$  & \todo{}  &  \todo{}   \\
		Proposed (dim knobs = 64) & $8.4$  & $0.62 \pm 0.15$  & \todo{}  &  \todo{}   \\
		\bottomrule
	\end{tabular}
\end{table}



\begin{table}
	\caption{\textbf{Experiment results --- speech (VCTK), nonparallel text.} The table shows the quantitative evaluation results on VCTK dataset. In the experiment, the style references are drawn from the validation set (unseen speakers) and have different contents from the target contents. }
	\label{table: vctk, valid, nonparallel}
	\def\tablewidth{18mm} 
	\centering
	\begin{tabular}{p{47mm}C{\tablewidth}C{\tablewidth}C{\tablewidth}C{\tablewidth}}
		\toprule
		Method     & Word-error rate (\%) $\downarrow$   \newline (real: 7.8) &  Cosine \newline similarity $\uparrow$  &  Mean opinion score (naturalness) $\uparrow$ &  Mean opinion score (similarity) $\uparrow$ \\
		\midrule
		Tacotron & $16.2$  & $0.03\pm 0.12$  & \todo{}  &  \todo{}   \\
		GST (\# tokens = 16)  & $16.0$  & $0.20 \pm 0.18$  &  \todo{} & \todo{}    \\
		GST (\# tokens = 64)  & $14.6$  & $0.18 \pm 0.16$  & \todo{}  &  \todo{}   \\
		GST (\# tokens = 16)  + embedding  & $12.0$  & $0.30 \pm 0.14$  & \todo{}  & \todo{}    \\
		GST (\# tokens = 64) + embedding & $16.0$  & $0.34 \pm 0.11$  &  \todo{}  & \todo{}    \\
		Proposed (dim knobs = 64) & $8.6$  & $0.44 \pm 0.14$  &  \todo{}  &  \todo{}   \\
		\bottomrule
	\end{tabular}
\end{table}




\begin{table}
	\caption{\textbf{Experiment results --- speech (LibriTTS-all-960), parallel text.} The table shows the quantitative evaluation results on LibriTTS dataset. In the experiment, the style references are drawn from the training set (seen speakers) and have the same content as the target content. }
	\label{table: libritts, train, parallel}
	\def\tablewidth{18mm} 
	\centering
	\begin{tabular}{p{47mm}C{\tablewidth}C{\tablewidth}C{\tablewidth}C{\tablewidth}}
		\toprule
		Method     & Word-error rate (\%) $\downarrow$ \newline (real: 6.3)  &  Cosine \newline similarity $\uparrow$  &  Mean opinion score (naturalness) $\uparrow$ &  Mean opinion score (similarity) $\uparrow$ \\
		\midrule
		Tacotron & $62.1$  & $-0.02 \pm 0.10$  &  \todo{}  &   \todo{}  \\
		GST (\# tokens = 16)  & $24.6$  & $0.12 \pm 0.18$  & \todo{}   &  \todo{}    \\
		GST (\# tokens = 64)  & $14.7$  & $0.24 \pm 0.16$  &  \todo{}  &  \todo{}   \\
		GST (\# tokens = 64) + embedding & $13.3$  & $0.50 \pm 0.19$  &  \todo{}  &  \todo{}   \\
		Proposed (dim knobs = 64) & $7.8$  & $0.76 \pm 0.10$  &  \todo{}  &  \todo{}   \\
		\bottomrule
	\end{tabular}
\end{table}

\begin{table}
	\caption{\textbf{Experiment results --- speech (LibriTTS-all-960), nonparallel text.} The table shows the quantitative evaluation results on LibriTTS dataset. In the experiment, the style references are drawn from the training set (seen speakers) and have different contents from the target contents. }
	\label{table: libritts, train, nonparallel}
	\def\tablewidth{18mm} 
	\centering
	\begin{tabular}{p{47mm}C{\tablewidth}C{\tablewidth}C{\tablewidth}C{\tablewidth}}
		\toprule
		Method     & Word-error rate (\%) $\downarrow$   \newline (real: 6.3) &  Cosine \newline similarity $\uparrow$  &  Mean opinion score (naturalness) $\uparrow$ &  Mean opinion score (similarity) $\uparrow$ \\
		\midrule
		Tacotron & $65.8$  & $-0.02 \pm 0.10$  &  \todo{}  &  \todo{}   \\
		GST (\# tokens = 16)  & $46.8$  & $0.00 \pm 0.10$  &  \todo{}  &  \todo{}   \\
		GST (\# tokens = 64)  & $32.8$  & $0.20 \pm 0.19$  &  \todo{}  &  \todo{}   \\
		GST (\# tokens = 64) + embedding & $18.4$  & $0.37 \pm 0.23$  &  \todo{}  &   \todo{}   \\
		Proposed (dim knobs = 64) & $5.9$  & $0.81 \pm 0.12$  &  \todo{}  &  \todo{}   \\
		\bottomrule
	\end{tabular}
\end{table}


\begin{table}
	\caption{\textbf{Experiment results --- speech (LibriTTS-all-960), nonparallel text.} The table shows the quantitative evaluation results on LibriTTS dataset. In the experiment, the style references are drawn from the validation set (unseen speakers) and have different contents from the target contents. }
	\label{table: libritts, valid, nonparallel}
	\def\tablewidth{18mm} 
	\centering
	\begin{tabular}{p{47mm}C{\tablewidth}C{\tablewidth}C{\tablewidth}C{\tablewidth}}
		\toprule
		Method     & Word-error rate (\%) $\downarrow$ \newline (real: 6.3)  &  Cosine \newline similarity $\uparrow$  &  Mean opinion score (naturalness) $\uparrow$ &  Mean opinion score (similarity) $\uparrow$ \\
		\midrule
		Tacotron & $62.6$  & $0.01 \pm 0.09$  &  \todo{}  &  \todo{}   \\
		GST (\# tokens = 16)  & $27.9$  & $0.07 \pm 0.12$  &  \todo{} &  \todo{}   \\
		GST (\# tokens = 64)  & $31.1$  & $0.08 \pm 0.13$  &  \todo{}  &   \todo{}   \\
		GST (\# tokens = 64) + embedding & $16.2$  & $0.26 \pm 0.15$  &  \todo{}  &  \todo{}   \\
		Proposed (dim knobs = 64) & $7.2$  & $0.56 \pm 0.15$  &  \todo{}  &  \todo{}   \\
		\bottomrule
	\end{tabular}
\end{table}

==> user_study.tex <==
\subsection{Qualitative Evaluation for Speech}
To qualitatively evaluate the style similarity of the generated sequence with reference input, we designed a simple user-study where users were given with pairs of referenced and synthesized audio and asked if ``the two samples could have been produced by the same speaker in a similar environmental condition." 
Following the protocol used by \citet{zhao2020voice}, users were given the following 4 choices and scores: `` 4 (Absolutely same)", ``3 (Likely same)", ``2 (Likely different)", ``1 (Absolutely different)". 
We randomly selected a subset of $100$ pairs of generated and reference audio samples and collected a total of $xx$ responses from $x$ participants.
The mean opinion score (MOS) for each algorithm is computed by averaging the scores from all the participants.
To find upper-bound on MOS, in our study we also mixed pairs of two real samples from the same speakers.
The average mean opinion score (MOS) (out of 4.0) is presented in the Table \todo{}

